MemSAC: Memory Augmented Sample Consistency for Large Scale Unsupervised Domain Adaptation

Practical real world datasets with plentiful categories introduce new challenges for unsupervised domain adaptation like small inter-class discriminability, that existing approaches relying on domain invariance alone cannot handle sufficiently well. In this work we propose MemSAC, which exploits sample level similarity across source and target domains to achieve discriminative transfer, along with architectures that scale to a large number of categories. For this purpose, we first introduce a memory augmented approach to efficiently extract pairwise similarity relations between labeled source and unlabeled target domain instances, suited to handle an arbitrary number of classes. Next, we propose and theoretically justify a novel variant of the contrastive loss to promote local consistency among within-class cross domain samples while enforcing separation between classes, thus preserving discriminative transfer from source to target. We validate the advantages of MemSAC with significant improvements over previous state-of-the-art on multiple challenging transfer tasks designed for large-scale adaptation, such as DomainNet with 345 classes and fine-grained adaptation on Caltech-UCSD birds dataset with 200 classes. We also provide in-depth analysis and insights into the effectiveness of MemSAC.

==> Tables/CUB200.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Own experiment values %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{wraptable}{r}{0.4\textwidth}
% \begin{wraptable}{r}{0.45\textwidth}
  \centering
   \captionsetup{width=0.4\textwidth, font=footnotesize}
  \caption{Results on fine-grained adaptation on 200 categories from CUB-Drawings dataset. Bold and underline indicate the best and second best methods respectively. $\dagger$Uses hierarchical label annotation.}
  \label{tab:cub200_result}
  \resizebox{0.4\textwidth}{!}{
%   \rowcolors{2}{gray!25}{white}
% \centering
% \small
  \begin{tabular}{@{} l *{6}{c} @{}} 
    \toprule  \\[-1em]
    Method & C $\rightarrow$ D && D $\rightarrow$ C && Avg. \\
    \midrule
    Resnet-50 & 60.88 && 42.07 && 51.47 \\
    MCD~\cite{saito2018maximum} & 50.18 && 38.56 && 44.37 \\
    % ADDA & 60.12 && 40.65 && 50.36 \\
    SAFN~\cite{xu2019larger} & 60.29 && 41.34 && 50.82 \\
    CAN~\cite{kang2019contrastive} & 52.18 && 50.05 && 51.11 \\
    RSDA~\cite{gu2020spherical} & 61.04 && 44.20 && 52.62 \\
    DANN~\cite{DANN} & 62.09 && 47.73 && 54.91 \\
    HDAN~\cite{cui2020hda} & 60.25 && 52.40 && 56.33 \\
    % MCC & 66.78 && 50.15 && 58.47 \\
    FixBi~\cite{na2021fixbi} & 68.20 && 49.47 && 58.84 \\
    CDAN~\cite{CDAN} & 68.12 && 53.83 && 60.98 \\
    ToAlign~\cite{wei2021toalign} & - && - && - \\
    PAN$\dagger$~\cite{PAN} & \underline{70.53} && \underline{55.38} && \underline{62.96}$\dagger$ \\
    \Ours & \textbf{71.78}  && \textbf{59.48}  && \textbf{65.63} \\
    \bottomrule
  \end{tabular}}
    % \vspace{-16pt}
%   \vspace{-16pt}
% \end{wraptable}
\end{wraptable}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Tables/CUB_Dnet126_OH.tex <==
\begin{table*}[!tbp]
\centering
% \makebox[0pt][c]{\parbox{0.98\textwidth}{%
    \begin{subtable}[t]{0.45\hsize}\centering
          \resizebox{\textwidth}{!}{
          \rowcolors{2}{gray!25}{white}
        % \centering
        % \small
          \begin{tabular}{@{} l *{6}{c} @{}} 
            \toprule  \\[-1em]
            Method & C $\rightarrow$ D && D $\rightarrow$ C && Avg. \\
            \midrule
            Resnet-50*~\cite{he2016deep} & 60.88 && 42.07 && 51.47  \\
            % DAN~\cite{long2015learning} & 58.95 && 39.33 && 49.14 \\
            DANN*~\cite{DANN} & 62.09 && 47.73 && 54.91 \\
            JAN~\cite{long2017deep} & 62.42 && 40.37 && 51.40 \\
            ADDA~\cite{tzeng2017adversarial} & 60.12 && 40.65 && 50.36 \\
            % MADA~\cite{pei2018multi} & 63.67 && 44.28 && 53.98 \\
            MCD*~\cite{saito2018maximum} & 50.18 && 38.56 && 44.37 \\
            SAFN*~\cite{xu2019larger} & 60.29 && 41.34 && 50.82 \\
            RSDA*~\cite{gu2020spherical} & 61.04 && 44.20 && 52.62 \\
            CDAN*~\cite{CDAN} & \underline{68.12} && \underline{53.83} && \underline{60.98} \\
            PAN*~\cite{PAN} & 70.53 && 55.38 && 62.96 \\
            \midrule
            \Ours & \textbf{71.78}$^{\pm 0.12}$  && \textbf{59.48}$^{\pm 0.22}$  && \textbf{65.63} \\
            \bottomrule
          \end{tabular}}
        %   \captionsetup{width=\textwidth, font=footnotesize}
          \caption{}
          \label{tab:cub200_result}
    \end{subtable}
    \hfill
    \begin{subtable}[t]{0.25\hsize}\centering
    \rowcolors{2}{gray!25}{white}
            \begin{tabular}{@{} l c c @{} }
                \toprule
                Method && Avg. Accuracy \\
                \midrule
                Resnet-50 && 49.20 \\
                % \midrule
                MCD~\cite{saito2018maximum} && 52.18 \\
                RSDA~\cite{gu2020spherical} && 53.44 \\
                DANN~\cite{DANN} && 56.90  \\
                BSP~\cite{chen2019transferability} && 55.06 \\
                % BSP+CDAN-E & 67.79  & 68.15 & 60.31 && 64.65 & 51.21 & 56.47 && 70.43 & 57.00 & 56.47 && 65.66 & 64.18 & 62.40 && 62.05 \\
                SAFN~\cite{xu2019larger} && 58.18 \\
                CDAN~\cite{CDAN} && 61.11 \\
                PAN~\cite{PAN}$^\dagger$ && \underline{61.75} \\
                \midrule
                \Ours{} && \textbf{64.76} \\ 
                \bottomrule
            \end{tabular}
            % \captionsetup{width=\textwidth, font=footnotesize}
            \caption{}
            \label{tab:domainnet126}
    \end{subtable}
    \hfill
    \begin{subtable}[t]{0.25\hsize}\centering
    \rowcolors{2}{gray!25}{white}
            \begin{tabular}{lcc}
            \toprule
            Method & AVG \\
            \midrule
            Resnet-50 & 46.1 \\
            \midrule
            DAN~\cite{long2015learning} & 56.3 \\
            DANN~\cite{DANN} & 57.6 \\
            JAN~\cite{long2017deep} & 58.3 \\
            CDAN~\cite{CDAN} & 65.8 \\
            BSP~\cite{chen2019transferability} & 66.3\\
            % MDD~\cite{zhang2019bridging} & \textbf{54.9} & \textbf{73.7} & \textbf{77.8} & 60.0 & \textbf{71.4} & 71.8 & 61.2 & \textbf{53.6} & 78.1 & \underline{72.5} & \textbf{60.2} & \underline{82.3} & 68.1 \\
            SAFN~\cite{xu2019larger} & \underline{67.3} \\
            % MCS & 55.9 & 73.8 & 79.0 & 57.5 & 69.9 & 71.3 & 58.4 & 50.3 & 78.2 & 65.9 & 53.2 & 82.2 & 66.3 \\      
            % InstaPBM~\cite{li2020rethinking} & 54.4 & 75.3 & 79.3 & \underline{65.4} & \textbf{74.2} & \textbf{75.0} & 63.3 & 49.7 & \underline{80.2} & \underline{72.8} & 57.8 & \underline{83.6} & \underline{69.7} \\              
            % MDD+I.A~\cite{jiang2020implicit} & \underline{56.2} & \textbf{77.9} & \underline{79.2} & 64.4 & \underline{73.1} & 74.4 & \underline{64.2} & \underline{54.2} & 79.9 & 71.2 & \underline{58.1} & 83.1 & 69.5 \\    
            \midrule
            \Ours{} & \textbf{68.42} \\
            \bottomrule
            \end{tabular}
            % }
            % \captionsetup{width=\textwidth, font=footnotesize}
            \caption{}
            \label{tab:officehome}
    \end{subtable}
\captionsetup{width=\textwidth, font=footnotesize}
\caption{Accuracy scores on (\ref{tab:cub200_result}) 200 classes from the CUB-birds dataset, (\ref{tab:domainnet126}) 126 classes from the DomainNet dataset, (\ref{tab:officehome}) 65 categories on OfficeHome~\cite{venkateswara2017deep} dataset. \textbf{Bold} and \underline{underline} denote the best and next best performing methods respectively. 
% Numbers for baselines taken from \cite{chen2019transferability} and \cite{xu2019larger}.
}
\label{tab:ablations}
\vspace{-8pt}
\end{table*}



==> Tables/FG_results.tex <==
\begin{table}[t]
    \begin{minipage}[b]{0.16\textwidth}
    \centering
        \resizebox{\textwidth}{!}{
        \begin{tabular}{@{} l *{3}{c} @{} }
            \toprule
            & {birds-123} & {CompCars}\\
            \midrule
            Source & 72.02 & 15.64 \\
            DANN & 63.36 & 48.90 \\
            PAN & 74.04 & 48.62 \\
            CDAN & 72.95 & 50.40 \\
            MemSAC & 78.42 & 52.75 \\
            \bottomrule
        \end{tabular}
        }
        \captionsetup{width=\textwidth, font=footnotesize}
        \caption{Finegrained accuracy}
        \label{tab:fgdata}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.14\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
        \begin{tabular}{@{} l *{3}{c} @{} }
            \toprule
            & \footnotesize{W/ kNN} & \footnotesize{Classifier PL}\\
            \midrule
            w/ Mem. & \textbf{47.26} & 44.81 \\
            w/o Mem. & 43.32 & 43.24 \\
            \bottomrule
        \end{tabular}
        }
        \captionsetup{width=\textwidth, font=footnotesize}
        \caption{Memory vs. kNN-PL} 
        \label{tab:memknn}
    \end{minipage}
    % \begin{minipage}[b]{0.19\textwidth}
    %     \centering
    %     \resizebox{\textwidth}{!}{
    %     \begin{tabular}{@{} l *{3}{c} @{} }
    %         \toprule
    %         & R-> C & all 12 tasks\\
    %         \midrule
    %         Source Only & 41.61 & 35.98 \\
    %         + MemSAC & 43.18(\textcolor{blue}{+1.57\%}) & 38.11(\textcolor{blue}{+2.13\%}) \\
    %         \midrule
    %         CDAN & 50.15 & 43.24 \\
    %         + MemSAC & 54.34(\textcolor{blue}{+4.19\%}) & 47.26(\textcolor{blue}{+4.02\%}) \\
    %         \bottomrule
    %     \end{tabular}
    %     }
    %     \captionsetup{width=\textwidth, font=footnotesize}
    %     \caption{tghr} 
    %     \label{tab:memknn}
    % \end{minipage}
    \begin{minipage}[b]{0.16\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
        \begin{tabular}{@{} l *{3}{c} @{} }
            \toprule
            & DomainNet \\
            \midrule
            Source Only & 35.98 \\
            + MemSAC & 38.11(\textcolor{blue}{+2.13\%}) \\
            \midrule
            CDAN & 43.24 \\
            + MemSAC & 47.26(\textcolor{blue}{+4.02\%}) \\
            \bottomrule
        \end{tabular}
        }
        \captionsetup{width=\textwidth, font=footnotesize}
        \caption{SourceOnly \Ours{}} 
        \label{tab:sourcemsac}
    \end{minipage}
    \vspace{-18pt}
\end{table}


==> Tables/dnet_small.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%  DomainNet-345 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[htbp]
    \begin{center} 
    \setlength{\tabcolsep}{3pt}
    \resizebox{\textwidth}{!}{
  \rowcolors{2}{gray!25}{white}
    \begin{tabular}{@{} l *{17}{c} @{} }
        \toprule
        Source & \multicolumn{3}{c}{\textbf{Real$\rightarrow$}} && \multicolumn{3}{c}{\textbf{Clipart$\rightarrow$}} && \multicolumn{3}{c}{\textbf{Painting$\rightarrow$}} && \multicolumn{3}{c}{\textbf{Sketches}$\rightarrow$} && \\
        \cline{2-4} \cline{6-8} \cline{10-12} \cline{14-16}
        Target & {C} & {P} & {S} && {R} & {P} & {S} && {R} & {C} & {S} && {R} & {C} & {P} && Avg. \\
        \midrule
        ResNet-50& 41.61& 42.79& 29.66& & 42.41& 27.24& 32.15& & 49.52& 32.55& 26.73& & 38.75& 40.89& 27.5& & 35.98 \\
        % MSTN~\cite{xie2018learning} & 27.25& 32.98& 24.35& & 28.17& 21.14& 24.15& & 30.74& 19.85& 22.5& & 24.31& 26.22& 23.56& & 25.44 \\
        % RSDA~\cite{gu2020spherical} & 27.28 & 35.83& 24.35& & 36.98& 24.94& 31.12& & 41.32& 26.1& 24.71& & 29.46& 26.22& 27.79& & 29.68 \\
        % BSP~\cite{chen2019transferability} & 34.51 & 39.14& 27.57& & 40.56& 26.71& 30.72& & 40.83& 24.56& 26.85& & 36.54& 32.37& 28.08 & & 32.37 \\
        MCD~\cite{saito2018maximum}$^\ddagger$ & 36.34& 36.58& 24.95& & 40.32& 25.83& 32.12& & 43.65& 29.66& 25.7& & 34.16& 39.11& 26.89& & 32.94$^\ddagger$ \\
        ILADA~\cite{ILA}$^\mathsection$ & 46.45 & 39.01 & 35.4&& 47.94 &26.68 &36.33 &&43.00 & 26.62 & 27.3 && 48.85 & 47.68 & 32.23 && 38.12$^\mathsection$  \\
        SAFN~\cite{xu2019larger} & 38.11& 45.96& 29.20 & & 45.96& 30.00 & 34.65& & \underline{54.44}& 34.74& 30.64& & 45.29& 47.43& 38.01& & 39.54 \\
        % DANN~\cite{DANN} & 45.93& 44.51& 35.47& & 46.85& 30.52& 36.77& & 48.02& 34.76& 32.15& & 47.1& 46.45& 38.47& & 40.58 \\
        CAN~\cite{kang2019contrastive}$^\mathsection$ & 40.71 &37.77 &33.7 && \textbf{54.93} &31.41 &37.37 && 51.05 &33.64 &30.95 && \underline{52.13} &42.19 &32.04 && 39.82$^\mathsection$  \\
        PAN~\cite{PAN}$^\dagger$ & 49.25 &48.18 &36.46 && 49.66 &33.27 &38.78 && 51.89 &36.01 &32.94 && 49.12 &50.94 &39.89 && 43.03 $^\dagger$ \\
        CDAN~\cite{CDAN} & 50.15& 48.35& 39.01& & 50.02& 33.39& 39.3& & 52.21& 36.44& 33.68& & 48.46& 49.27& 38.65& & 43.24 \\
        HDAN~\cite{cui2020hda} & 46.30 & 47.52 & 34.39 & & 49.91 & 33.98 & 37.98 & & \textbf{55.26} & \textbf{40.82} & 32.77 & & 49.04 & 49.77 & 40.04 & & 43.15 \\
        FixBi~\cite{na2021fixbi}$^\ddagger$ & \underline{51.18}& \underline{49.19}& \underline{39.65}& & 50.02& \underline{34.59}& \underline{41.17}& & 52.21& 36.44& \underline{33.68}& & 50.84& \underline{53.51}& \underline{41.67}& & \underline{44.51}$^\ddagger$ \\
        \midrule
        % MemSAC+CAN & 43.79$^{\pm.46}$& 38.99$^{\pm.17}$& 36.71$^{\pm.23}$& & 55.36$^{\pm.06}$& 32.41$^{\pm.09}$& 39.46$^{\pm.11}$& & 52.48$^{\pm.18}$& 35.21$^{\pm.32}$& 32.89$^{\pm.14}$& & 54.15$^{\pm.06}$& 44.60$^{\pm.06}$& 33.02$^{\pm.22}$& & 41.59 \\
        MemSAC [Ours] & \textbf{54.34}& \textbf{52.27}& \textbf{41.74}& & \underline{54.4}& \textbf{36.67}& \textbf{42.15}& & 53.24& \underline{40.39}& \textbf{37.22}& & \textbf{53.03}& \textbf{54.31}& \textbf{44.56}& & \textbf{47.03} \\
        \midrule
        % \midrule
        % Tgt. Supervised & 72.59 & 62.66 & 65.12 & & 80.92 & 62.66 & 65.12 & & 80.92 & 72.59 & 65.12 & & 80.92 & 72.59 & 62.66 & & 70.32 \\
        \bottomrule
        \end{tabular}}
    \end{center}
    \vspace{-16pt}
    % \captionsetup{width=\textwidth, font=footnotesize}
    \caption{Accuracy scores on \dnet-345 using Resnet-50 backbone. Best values are in \textbf{bold} and the next best are \underline{underlined}. \Ours{} performs better than all other methods on most of the tasks. $^\dagger{}$Uses hierarchical label annotation. $^\ddagger$prediction uses ensemble classifiers. $^\mathsection$Uses class-balanced sampling.}
    \label{tab:domainnet345}
    \vspace{-12pt}
\end{table*}

==> Tables/inference_times.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% Different ablation %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table}[!tbp]
\centering

    \resizebox{0.4\textwidth}{!}{
        \begin{tabular}{@{} l *{3}{c} @{} }
            \toprule
            Method & Peak GPU Mem. & Training Time & Avg. Acc\\
            \midrule
            DANN & 7.9GB & 11.7 Hrs & 40.58\% \\
            CDAN & 8.2GB & 12 Hrs & 43.24\% \\
            \Ours{} & 8.5GB & 12.63 Hrs & 47.03\% \\
            \bottomrule
        \end{tabular}
        }
    \captionsetup{width=0.5\textwidth, font=footnotesize}
    \caption{\Ours{} adds negligible memory and time overhead to the training even with large queues, and zero overhead during inference.} 
    \label{tab:inftime}
\vspace{-8pt}

\end{table}

==> scripts/acc_vs_levels.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Hierarchy and simscores %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!t]
     \centering
     \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/HierarchyAcc.pdf}
        \captionsetup{width=0.95\textwidth, font=footnotesize}
        \caption{Comparison of accuracy vs. granularity of labels on \textbf{C}$\rightarrow$\textbf{D} and \textbf{D}$\rightarrow$\textbf{C} on CUB-Drawings dataset for 4 levels of label hierarchy. }
        \label{fig:hierarchyAcc}
     \end{minipage}
     \hfill
    \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/domainNetClasses.pdf}
        \captionsetup{width=0.98\textwidth, font=footnotesize}
        \caption{\textit{Gain in accuracy} ($\Delta$) over a model trained only on source data, using various adaptation approaches vs. the \#classes from \dnet{} for \textbf{R}$\rightarrow$\textbf{C}.
        }
        \label{fig:dnetClasses}
     \end{minipage}
     \hfill
     \begin{minipage}[t]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/SimScores.pdf}
        \captionsetup{width=0.95\textwidth, font=footnotesize}
        \caption{Mean similarity score for \emph{within-class} samples vs. training iteration shown for \textbf{D}$\rightarrow$\textbf{C} on CUB-Drawings.
        }
        \label{fig:simScores}
     \end{minipage}
\vspace{-0.3cm}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
